SMATE: Semi-Supervised Spatio-Temporal Representation Learning on Multivariate Time Series

Learning from Multivariate Time Series (MTS) has attracted widespread attention in recent years. In particular, label shortage is a real challenge for the classification task on MTS, considering its complex dimensional and sequential data structure. Unlike self-training and positive unlabeled learning that rely on distance-based classifiers, in this paper, we propose SMATE, a novel semi-supervised model for learning the interpretable Spatio-Temporal representation from weakly labeled MTS. We validate empirically the learned representation on 30 public datasets from the UEA MTS archive. We compare it with 13 state-of-the-art baseline methods for fully supervised tasks and four baselines for semi-supervised tasks. The results show the reliability and efficiency of our proposed method.

==> model_param_nbr.tex <==
% \usepackage{caption}
\begin{table}[!htbp]
\centering
\vspace{-0.5em}
%\captionsetup{labelformat=empty}
\caption{Parameter numbers of deep learning models on MTSC}
\vspace{-0.5em}
\label{model_param_nbr}
\scalebox{0.85}{
\begin{tabular}{|l|c|c|c|c|c|} 
\hline
    \textit{ArticularyWordR.} & SMATE  & MLSTM-FCN & CA-SFCN & USRL   & TapNet  \\ 
\hline
Param. number & 564585 & 597865    & 685965 & 368655 & 635285  \\
\hline
\end{tabular}
}
\vspace{-1em}
\end{table}
